A Methodology for Player Modeling based on Machine Learning

AI is gradually receiving more attention as a fundamental feature to increase the immersion in digital games. Among the several AI approaches, player modeling is becoming an important one. The main idea is to understand and model the player characteristics and behaviors in order to develop a better AI. In this work, we discuss several aspects of this new field. We proposed a taxonomy to organize the area, discussing several facets of this topic, ranging from implementation decisions up to what a model attempts to describe. We then classify, in our taxonomy, some of the most important works in this field. We also presented a generic approach to deal with player modeling using ML, and we instantiated this approach to model players' preferences in the game Civilization IV. The instantiation of this approach has several steps. We first discuss a generic representation, regardless of what is being modeled, and evaluate it performing experiments with the strategy game Civilization IV. Continuing the instantiation of the proposed approach we evaluated the applicability of using game score information to distinguish different preferences. We presented a characterization of virtual agents in the game, comparing their behavior with their stated preferences. Once we have characterized these agents, we were able to observe that different preferences generate different behaviors, measured by several game indicators. We then tackled the preference modeling problem as a binary classification task, with a supervised learning approach. We compared four different methods, based on different paradigms (SVM, AdaBoost, NaiveBayes and JRip), evaluating them on a set of matches played by different virtual agents. We conclude our work using the learned models to infer human players' preferences. Using some of the evaluated classifiers we obtained accuracies over 60% for most of the inferred preferences.

==> abstract.tex <==
Artificial Intelligence (AI) is gradually receiving more attention as a fundamental feature to increase the immersion in digital games. Among the several AI approaches, player modeling is becoming an important one. The main idea is to understand and model the player characteristics and behaviors in order to develop a better AI. It is possible to model player aspects in different levels of abstraction, such as actions, position, preferences, knowledge and satisfaction. This modeling allows games to customize their AI, difficulty or levels to specific players, making the game experience more interesting.

In this work, we discuss several aspects of this new field. Since several works have been tackling this problem, we proposed a taxonomy to organize the area, discussing several facets of this topic, ranging from implementation decisions up to what a model attempts to describe. We then classify, in our taxonomy, some of the most important works in this field. Besides the taxonomy, we also presented a generic approach to deal with player modeling using machine learning, and we instantiated this approach to model players' preferences in the game \textsc{Civilization IV}.

The instantiation of this approach has several steps. We first discuss a generic representation, regardless of what is being modeled, and evaluate it performing experiments with the strategy game \textsc{Civilization IV}. Results show the effectiveness of this representation in characterizing and modeling agents.

Continuing the instantiation of the proposed approach we evaluated the applicability of using game score information to distinguish different preferences. To perform this task we presented a characterization of virtual agents in the game, comparing their behavior with their stated preferences. Once we have characterized these agents, we were able to observe that different preferences generate different behaviors, measured by several game indicators. Using this information we tackled the preference modeling problem as a binary classification task, with a supervised learning approach. We compared four different methods, based on different paradigms (\textit{SVM}, \textit{AdaBoost}, \textit{NaiveBayes} and \textit{JRip}), evaluating them on a set of matches played by different virtual agents. We obtained accuracies that improved by far the state of the art. We conclude our work using the learned models to infer human players' preferences. Using some of the evaluated classifiers we obtained accuracies over 60\% for most of the inferred preferences.

==> agradecimentos.tex <==
Since most of the people I am acknowledging here speak Portuguese, and not necessarily English, I am going to present my acknowledgments in Portuguese, once this text is for them. The unique exception is Pieter Spronck, who I am thankful for kindly sharing his dataset, source code and impressions with me.\\

Quando eu comecei o mestrado, pensava que n\~ao teria muitas pessoas para agradecer ao final. Achava que agradeceria somente aos meus pais, orientadores, irm\~ao e noiva. Eu estava errado, sou grato a muitas outras pessoas.

Primeiro, referente \`a minha fam\'ilia, eu gostaria de agradecer aos meus pais, que sempre, incondicionalmente, me incentivaram a fazer o mestrado. Al\'em deles, uma pessoa extremamente presente em todo esse per\'iodo foi meu irm\~ao, que me ouviu, assistiu pr\'evias de palestras, leu peda\c{c}os de artigos, sempre disposto a dar opini\~ao. Muito obrigado! Tamb\'em sou muito grato \`a minha futura fam\'ilia: Poliana. Obrigado por ter me ouvido, apoiado, e estado presente em cada dia desses dois anos. Por ter atendido minhas liga\c{c}\~oes, ap\'os reuni\~oes, para ouvir o que certamente n\~ao a interessava; e, principalmente, por ter acreditado em mim quando disse que casar\'iamos ap\'os o mestrado (j\'a est\'a marcado!) e por ter aceitado viver o meu sonho comigo! 

Al\'em da minha fam\'ilia, muitos amigos participaram, de alguma forma, desse mestrado. Agrade\c{c}o ao Rabelo, por ter escutado, diariamente, relat\'orios sobre o andamento de tudo. Gl\'ivia, Nat\'alia, Luiz, Denise, pelas risadas durante as visitas e caf\'es da tarde. Vitor, pelas longas conversas no \emph{gTalk}, sobre pesquisa, planejamentos, posts e rankings. N\~ao posso tamb\'em n\~ao mencionar meus co-autores, Bruno, Fantini e Renato, sem voc\^es, tudo teria sido mais dif\'icil.

Ainda relacionado \`as minhas publica\c{c}\~oes, gostaria de agradecer a todos os meus revisores ``secretos'', que certamente melhoraram a qualidade desse trabalho. Al\'em deles, ao Luiz, Gisele, Meira, Capes, CNPq e ao PPGCC, que viabilizaram minhas viagens nesses dois anos.

N\~ao h\'a como n\~ao agradecer tamb\'em ao Synergia, como um todo, pelo excelente ambiente de trabalho e flexibilidade de hor\'ario, o que facilitou imensamente o mestrado e permitiu que eu apresentasse meus artigos ao longo desses dois anos.

Gostaria de agradecer tamb\'em a todos os professores, da gradua\c{c}\~ao e mestrado que, de alguma forma, ajudaram nesse processo. Assim como todas as pessoas que foram parte dos meus experimentos, jogando \textsc{Civilization IV} com extrema boa vontade.

E por \'ultimo, mas de forma alguma menos importantes, meus dois orientadores: Luiz e Gisele. N\~ao h\'a como n\~ao ser grato a toda a aten\c{c}\~ao despendida pelo Luiz (70 reuni\~oes registradas e muitas outras ``passadas na sala'' sem registro!), conversas, paci\^encia e ensinamentos. Assim como a Gisele, que ``chegou depois'', mas a quem dei bastante trabalho e visitei bastante. Sou realmente muito grato a voc\^es!

Para concluir, tenho muita dificuldade em diferenciar o processo de aplica\c{c}\~ao do doutorado com a conclus\~ao do mestrado. Por isso, gostaria de agradecer a todos que se propuseram a me auxiliar, de alguma forma, nesse processo. Luiz Chaimowicz, Gisele Pappa, Wagner Meira, Antonio Loureiro, Nivio Ziviani, Jussara Almeida, Adriano Veloso, Marisa Mancini, Mario Nascimento e toda a Secretaria do DCC, muito obrigado. 

Eu certamente sentirei saudades do DCC!

==> dedicatoria.tex <==
Dedico este trabalho aos meus pais, Marlos e Michelle. Essa \'e, de certa forma, tamb\'em a realiza\c{c}\~ao de seus sonhos.


==> resumo.tex <==
A Inteligência Artificial (IA) está recebendo cada vez mais atenção como uma característica fundamental para aumentar a imersão em jogos digitais. Entre as diversas abordagens de IA, uma que está se tornando importante é a modelagem de jogadores.  A principal ideia é entender e modelar as características e comportamentos de jogadores para o desenvolvimento de uma IA melhor. A modelagem de diferentes aspectos de jogadores é possível em diferentes níveis de abstração, como ações, posições, preferências e satisfação. Essa modelagem permite que jogos customizem sua IA, dificuldade ou fases, para jogadores específicos, criando uma experiência de jogo mais interessante.

Nesse trabalho, nós discutimos vários aspectos dessa nova área. Primeiramente, uma vez que diversos trabalhos têm abordado esse problema, nós propusemos uma taxonomia para organizar esse campo, discutindo diferentes facetas desse tópico, desde decisões de implementação até o que o mo\-de\-lo tenta descrever. Classificamos então, na nossa taxonomia, alguns dos trabalhos mais importantes nessa área.  Além da taxonomia, apresentamos também uma abordagem genérica para a mo\-de\-la\-gem de jogadores utilizando aprendizado de máquina, e instanciamos essa abordagem no problema de modelagem de preferências de jogadores no jogo \textsc{Civilization IV}.

A instanciação dessa abordagem passa por diversas etapas. Discutimos uma representação genérica, independentemente do que estiver sendo modelado, e a avaliamos rea\-li\-zan\-do experimentos com o jogo de estratégia \textsc{Civilization IV}. Resultados mostram a efetividade de caracterização e modelagem dessa abordagem. 

Continuando a instanciação da abordagem proposta, avaliamos a aplicabilidade de se utilizar informações de pontuações de jogadores para distinguir diferentes pre\-fe\-rên\-cias. Para isso apresentamos uma caracterização de agentes virtuais no jogo, comparando seu comportamento com as suas preferências pré-definidas no código-fonte. Uma vez que caracterizamos esses agentes, fomos capazes de observar que diferentes preferências geram diferentes comportamentos. Usando essas informações, atacamos o problema de modelagem de preferências como uma tarefa de classificação binária, com uma abordagem de aprendizado supervisionado. Nós comparamos quatro métodos diferentes, baseados em diferentes paradigmas (\textit{SVM}, \textit{AdaBoost},  \textit{NaiveBayes} e \textit{JRip}), avaliando-os em um conjunto de partidas jogadas por diferentes agentes virtuais. Atingimos acurácias que superam largamente o estado da arte. Concluindo nosso trabalho, utilizamos os modelos aprendidos para inferir as preferências de jogadores humanos. Utilizando alguns dos classificadores avaliados, obti\-ve\-mos acurácias acima de 60\% para a maioria das preferências avaliadas.

